Scenario-based Probing and Steering Cultural Values in Large Language Models--Extended Version

Large Language Models (LLMs) are deployed across cultural contexts but often reflect homogenized values inherited from training data. Evaluations of cultural alignment typically rely on direct prompting with survey-style questions, which frequently elicit neutral or safety-aligned responses and fail to capture underlying model preferences. We propose a framework for probing and steering latent cultural representations in LLMs along the two Inglehart--Welzel axes of the World Values Survey (WVS). By translating social value questions into scenario-based behavioral dilemmas, we extract token-level probabilities to measure implicit values and apply activation steering, optionally combined with country-conditioned prompting, to shift model behavior without retraining. Across three open-source LLMs and four target cultures, we find substantial variation in steerability and identify latent entanglement, where interventions along one cultural dimension induce shifts along another. This coupling mirrors correlations in human WVS data and persists across activation, prompt, and hybrid steering. It constrains axis-independent alignment, though general task performance is largely preserved.

==> data/perplexity/plot.tex <==
% Perplexity vs Steering Coefficient figure
% Reads data from perplexity.csv (must be in the same directory as main.tex,
% or adjust the path in each \addplot table{...} below).
%
% Requires in main.tex preamble:
%   \usepackage{pgfplots}
%   \pgfplotsset{compat=1.18}
%   \usepackage{tikz}
%
% Import in main.tex with:
%   \begin{figure}[ht]
%     \centering
%     \input{perplexity_figure.tex}
%     \caption{Perplexity Change with Different Steering Coefficients}
%     \label{fig:perplexity}
%   \end{figure}

\begin{tikzpicture}
\begin{axis}[
    width=\linewidth,
    height=0.6\linewidth,
    title={Perplexity Change with Different Steering Coefficients},
    xlabel={Steering Coefficient},
    ylabel={Perplexity},
    xtick={-1.0,-0.8,-0.6,-0.4,-0.2,0.0,0.2,0.4,0.6,0.8,1.0},
    xticklabel style={font=\scriptsize},
    grid=both,
    grid style={dashed, gray!30},
    legend style={
        at={(0.02,0.98)},
        anchor=north west,
        legend columns=2,
        font=\scriptsize,
        fill=white,
        fill opacity=0.8,
        draw opacity=1,
        text opacity=1,
    },
    legend cell align={left},
    cycle list name=color list,
]

\addplot+[mark=*]         table[x=Steering Coefficient, y=X axis for Qwen,  col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{X axis for Qwen}

\addplot+[mark=square*]   table[x=Steering Coefficient, y=X axis for Llama, col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{X axis for Llama}

\addplot+[mark=triangle*] table[x=Steering Coefficient, y=X axis for Gemma, col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{X axis for Gemma}

\addplot+[mark=diamond*]  table[x=Steering Coefficient, y=Y axis for Qwen,  col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{Y axis for Qwen}

\addplot+[mark=pentagon*] table[x=Steering Coefficient, y=Y axis for Llama, col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{Y axis for Llama}

\addplot+[mark=otimes*]   table[x=Steering Coefficient, y=Y axis for Gemma, col sep=comma] {data/perplexity/perplexity.csv};
\addlegendentry{Y axis for Gemma}

\end{axis}
\end{tikzpicture}

==> revised_sections/abstract_new.tex <==
\begin{abstract}
Large Language Models (LLMs) are deployed across cultural contexts but often reflect homogenized values inherited from training data. Evaluations of cultural alignment typically rely on direct prompting with survey-style questions, which frequently elicit neutral or safety-aligned responses and fail to capture underlying model preferences. We propose a framework for probing and steering \emph{latent cultural representations} in LLMs along the two Inglehart--Welzel axes of the World Values Survey (WVS). By translating social value questions into scenario-based behavioral dilemmas, we extract token-level probabilities to measure implicit values and apply activation steering, optionally combined with country-conditioned prompting, to shift model behavior without retraining.
Across three open-source LLMs and four target cultures, we find substantial variation in steerability and identify \emph{latent entanglement}, where interventions along one cultural dimension induce shifts along another. This coupling mirrors correlations in human WVS data and persists across activation, prompt, and hybrid steering. It constrains axis-independent alignment, though general task performance is largely preserved.
\end{abstract}

==> sections/abstract.tex <==
\begin{abstract}
Large Language Models (LLMs) often exhibit homogenized cultural perspectives. While the World Values Survey (WVS) provides a gold standard for mapping human values, traditional direct prompting of LLMs on WVS often fails to access the model's latent cultural depth, leading to safety-aligned refusals or neutral responses. Here, we propose a generalizable framework for cultural evaluation and intervention that transitions from abstract queries to \textit{scenario-based behavioral probing}. By extracting implicit token probabilities across 300 situational dilemmas, we bypass surface-level alignment to map the latent coordinates of LLMs cultural value. We further introduce activation steering to shift these internal alignments during the forward pass without retraining. Our results reveal that cultural adaptability is non-uniform. While Llama exhibits structural rigidity, Qwen and Gemma show high but volatile sensitivity across social domains such as family and the legal system. Finally, we quantify \textit{latent entanglement}, demonstrating that models encode cultural axes as coupled ``modernization'' dimensions. This work establishes a computationally efficient framework for cultural steering, highlighting the structural complexities when navigating global value with LLMs.
\end{abstract}

==> sections/conclusion.tex <==
\section{Conclusion}

We proposed a framework for probing and steering latent cultural representations in LLMs. By translating abstract sociological questions into scenario-based behavioral dilemmas and analyzing token-level probabilities, we move beyond direct survey-style prompting, which often produces neutral or safety-aligned responses. We further showed that activation steering can shift cultural alignment without retraining, providing a lightweight mechanism for intervention at the representation level. The experiments reveal that cultural alignment is highly model-dependent, with clear differences in steerability across architectures. More importantly, we consistently observe latent entanglement: interventions targeting one cultural dimension also induce shifts along another. This suggests that cultural values are not encoded as independent axes, but as coupled latent structures, which limits the precision of fine-grained control. Our findings highlight both the potential and the limitations of cultural steering in LLMs, and suggest that future alignment methods must account for the geometry of internal representations rather than relying on prompting alone.



==> sections/ethics.tex <==
\section{Ethical Considerations}
Our work builds on the existing WVS questionnaire and employs open-source models and frameworks. While the constraining setup can be subjectively used to generate extreme steering behaviour, in the new scenario-based dataset we generate, we manually check for the removal/paraphrasing of any toxic language. The final situation questions and options are framed in a neutral tone. 


==> sections/experiments.tex <==
\section{Results and Discussion}
Across three architectures, scenario-based probing exposes culturally relevant representations that direct prompting fails to elicit, and hybrid steering---but not prompt-only steering---reliably shifts these representations toward non-Western targets while preserving general task performance. We develop this finding by first comparing evaluation paradigms (scenario-based vs.\ direct prompting), then reporting vector and hybrid steering results, examining the latent entanglement phenomenon, analyzing cross-domain robustness, and concluding with an assessment of task performance. The LLMs studied are \textbf{Llama 3.2-3B-Instruct} (28 layers), \textbf{Qwen3-4B-Instruct} (36 layers), and \textbf{Gemma3-4B} (34 layers), and we report results against four target cultures spanning the Inglehart--Welzel map: \textbf{Denmark}, \textbf{India}, \textbf{Mexico}, and \textbf{Vietnam}. Our experimental setup is detailed in Appendix \ref{app:exp_setup}\footnote{Code and dataset will be made available upon acceptance.}.

\subsection{Analysis of Evaluation Paradigms}
The comparison in Figure \ref{fig:reproduced_map} reveals a stark discrepancy. Using the direct explicit prompt of WVS (Figure \ref{fig:reproduced_map}, leftmost panel), models default largely to Western-centric clusters in the upper-right quadrant. With explicit prompting, Llama's refusal rate is 10\% with basic prompting, rising to 30\% with advanced persona-driven prompts. While the Qwen responds to all queries, it demonstrates a different form of output neutrality; 40\% of its responses are fixed at a safety score (5-6/10) and remain unchanged regardless of the culture-adapting instruction. \emph{The deviations across models, despite their comparable parameter counts, suggest that variations in pre-training data and architectural design play a decisive role in shaping cultural priors more than scale alone.}

On the other hand, when evaluated through our scenario-based behavioral probing (Figure \ref{fig:reproduced_map}, per-model panels), all three models exhibit a more pronounced alignment with secular-rational and self-expression values than in the explicit prompting setup. We also quantify this deviation and preference for scenario-based prompting by measuring the Euclidean distance from human data in WVS (see Appendix \ref{app:l2_distance} for details). \emph{Succinctly, situational dilemmas serve as a key to bypass default rigidity and achieve a more accurate positioning that reflects the nuanced reality of non-Western cultural representations.}

Comparing the two prompt-based conditions, Advanced Prompt Steering consistently yields a lower Euclidean distance to human WVS coordinates than Basic Prompt Steering across all three models, with the largest gaps observed for Vietnam and India---suggesting that the necessary cultural information exists within the models but is only accessible through high-fidelity instructions, particularly for non-Western cultures. Yet prompt conditioning alone has clear limits: Holm-corrected bootstrap tests in Appendix~\ref{app:l2_distance} show no significant distance reduction for Llama under prompt-only steering on any of the four target countries. For the most rigid architectures, activating culturally encoded representations requires direct intervention at the latent level, which motivates the layer-targeted vector steering approach we examine next.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{charts/layer_selection_line.png}
    \caption{The highest steering average differential per question when applying layer grid search vector steering. The questions are referenced in Tab.~\ref{tab:wvs_dimensions}.}
    \label{fig:layer_selection}
\end{figure}

\subsection{Vector Steering}
Figure \ref{fig:layer_selection} illustrates the steering differential across layers when applying vector steering Equation \ref{eq:situation_constrast} without including any cultural prompting. Our analysis reveals that cultural value information is encoded in specific, relatively early-to-mid stages of the transformer block. Specifically, layers \textbf{(16, 17, 18, 19)} for Qwen, \textbf{(8, 9, 11, 12)} for Llama, and \textbf{(12, 13, 14, 15)} for Gemma had the greatest influence on behavioral output.

The difference in magnitude of the shifts in Figure~\ref{fig:layer_selection} highlights a clear disparity in model flexibility and axis-specific sensitivity. Qwen appears significantly more malleable, with 8 out of 10 cultural questions meeting the threshold in Table~\ref{tab:wvs_dimensions}, while Llama shows greater stability or rigidity, with only 3 of 10 questions meeting that threshold. Here, Qwen shows moderate, balanced sensitivity across both axes, with several questions $X04$, $X05$ (``Caution regarding trusting people''), $Y02$ (``Priority on obedience/faith over independence'') maintaining a differential above $0.25$. In contrast, as expected, Llama exhibits the highest architectural rigidity; its steering differentials are the lowest among the three models, with most questions---and the model average---falling short of the $0.25$ threshold. This confirms our earlier findings from prompt-based steering that Llama possesses a stronger internal prior that resists external value modification. Meanwhile, Gemma demonstrates the highest malleability, particularly on the Survival vs. Self-Expression ($X$) axis, where question $X04$ (``Would not sign a political petition.'') exhibits a steering differential near $2.0$, and the model average consistently remains above $0.5$ across the targeted layers. Having identified architecture-specific sensitive layers, we next examine whether augmenting these activation vectors with prompt conditioning yields more precise cultural alignment.

\subsection{Hybrid Steering}
\label{subsec:hybrid_results}
We evaluate whether the hybrid configurations introduced in Section~\ref{subsec:hybrid_steering} yield more precise cultural alignment than either method alone. The per-model panels in Figure~\ref{fig:reproduced_map} overlay all steering configurations, while the bottom bar charts quantify the Euclidean distance from empirical human WVS coordinates.

Across all three models, hybrid steering reduces the average Euclidean distance from human coordinates relative to both prompt-only and vector-only baselines. However, the nature of this improvement is architecture-dependent, revealing three distinct interaction modes. For \textbf{Llama}, hybrid steering primarily redirects the cultural shift toward different quadrants while the magnitude remains small, confirming that structural rigidity limits displacement regardless of intervention type. For \textbf{Gemma}, hybrid steering amplifies magnitude along trajectories that remain parallel to the base vector direction in Figure~\ref{fig:steering_culture_map}, acting as a scalar amplifier rather than a directional modifier. \textbf{Qwen} uniquely modifies both direction and magnitude, departing from its base trajectory and sweeping a distinct path under hybrid conditioning, consistent with its compositional integration of prompt priors and latent directions.

A further distinction emerges between the two hybrid setups. For Llama and Gemma, Setup~1 ($v_L$) and Setup~2 ($v_L^{sp}$) produce nearly identical coordinates, suggesting that their latent representations are insensitive to the conditioning context of the contrastive pairs. In contrast, Qwen clearly distinguishes between setups, with the prompt-informed vector $v_L^{sp}$ yielding more distinct country-specific trajectories. The Holm-corrected bootstrap test in Appendix~\ref{app:l2_distance} corroborates this asymmetry: Hybrid~1 steering is significant on all model--country pairs except Gemma for Denmark. Across both steering regimes, however, interventions targeting one cultural axis consistently induce shifts along the other---a systematic coupling we now characterize.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{charts/steer_result_vector_line.png}
    \caption{Steering trajectory curves on the Inglehart-Welzel Cultural Map
    as $\alpha$ varies. Dashed and solid curves denote steering along the $X$
    and $Y$ axes respectively. The curves exhibit diminishing displacement at
    higher $\alpha$, saturating near $\alpha \in [0.5,0.6]$. The near-overlap of these curves across all
    three models reflects latent entanglement, while the qualitatively distinct
    trajectory shapes reveal architecture-dependent steerability.}
    \label{fig:steering_culture_map}
\end{figure}

\subsection{Latent Entanglement}
\label{sec:entanglement}

To evaluate the precision of our scenario-based latent steering, we apply the 300 optimized steering vectors to the 300 test scenarios. Ideally, an intervention along a single axis should result in an orthogonal shift. However, we consistently observe in Figures \ref{fig:reproduced_map} and \ref{fig:steering_culture_map} a phenomenon we term \textit{latent entanglement}, in which steering along one dimension produces an unintentional shift along the other.

Inspired by metrics for disentangled representation learning \cite{DBLP:conf/iclr/HigginsMPBGBML17}, we quantify this effect using the entanglement ratio ($E$) that measures the isolation of cultural dimensions within the latent space. The domain of $E$ is $[0, \infty)$, where $E = 0$ represents perfect orthogonality (ideal decoupling) and $E \geq 1$ indicates that the unintended shift meets or exceeds the intended intervention. Specifically, let $\Delta d_{\text{intended}}$ be the coordinate change along the targeted axis, i.e., the axis under consideration, and $\Delta d_{\text{unintended}}$ be the change along the non-targeted axis. For all $|\Delta d_{\text{intended}}| > 0$, the ratio is defined as Equation \ref{eq:entangle_score}:
\begin{equation}
E = \frac{|\Delta d_{\text{unintended}}|}{|\Delta d_{\text{intended}}|}
\label{eq:entangle_score}
\end{equation}

\input{tables/entanglement}

Table~\ref{tab:entanglement_ratio} reports $E$ across the three models and four domain partitions for both steering setups. First, entanglement is pervasive but not uniform: aggregate $E_{\text{All}}$ lies in $[0.72, 0.81]$ under vector-only steering, indicating that no model achieves orthogonal control, while the per-domain spread (Llama's $E_{\text{Legal}}=0.52$ vs.\ Gemma's $0.77$) shows that the strength of coupling depends on the social context being steered. Second, hybrid steering reduces entanglement, with the largest gains on the most rigid model: Llama drops from $0.72$ to $0.53$ on aggregate and from $0.52$ to $0.36$ in the legal domain, suggesting that prompt-informed vector extraction disentangles axes that pure activation contrasts fail to separate; Qwen shows a similar but smaller effect on the Family and Legal domains, while Gemma's aggregate is largely unchanged. Finally, the Workplace domain remains the most entangled across all models and both methods ($E_{\text{Workplace}} \in [0.73, 0.89]$), anticipating the cross-domain finding in Section~\ref{sec:domain} that professional norms behave as a coupled latent feature resistant to disentangling interventions. Latent entanglement is therefore not a monolithic property, but a domain-stratified one that hybrid steering only partially mitigates.

Across our experiments, we observed the near-complete overlap of the $X$- and $Y$-axis curves in Figure~\ref{fig:steering_culture_map} provides direct visual confirmation:
\emph{Interventions targeting opposite cultural axes trace virtually
indistinguishable paths}, and this degeneracy holds symmetrically across both
positive and negative $\alpha$. The $E$ values of $0.7$--$0.9$ quantify this
overlap numerically. Rather than an algorithmic artifact, this high entanglement serves as a critical validation of the model's latent mapping to human data.

To contextualize these values, we note that in empirical WVS data, the Traditional vs.\ Secular-Rational and Survival vs.\ Self-Expression axes are themselves correlated at $r=0.474$ across national means, confirming that these dimensions are not orthogonal in human populations either. The high $E$ values we observe thus mirror this real-world coupling: just as human societies rarely shift along one axis without a concurrent shift along the other, the model's latent space encodes these axes as co-dependent rather than independent. This suggests the model has internalized these human sociological dependencies as a single, unified latent feature.
Consistent with the modernization theory of \citet{inglehart2000modernization}, these two axes are fundamentally coupled in human societies; economic development typically triggers a simultaneous shift toward both self-expression and secular-rational authority. The magnitude of this entanglement, however, is not uniform: it varies markedly across the social domains we probe, as we now examine.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{charts/domain_heatmap_full2.png}
    \caption{Domain-wise shift on cultural axes when applying a steering vector along the $X$-axis at $\alpha=0.2$. Rows represent the source domain used to derive the steering vector, while columns represent the target domain where the shift is evaluated.}
    \label{fig:domain_heatmap}
\end{figure}

\subsection{Domain Analysis}
\label{sec:domain}
To assess the robustness of our method, we control for steering across the 3 distinct social domains: family, legal, and workplace. Figure \ref{fig:domain_heatmap} illustrates the shifts induced by $X$-axis steering at $\alpha=0.2$ across both the $X$-axis (Survival vs.\ Self-Expression) and the $Y$-axis (Traditional vs.\ Secular-Rational).

Our results reveal that Gemma is the most sensitive to domain-specific context, which aligns with our previous examination of Gemma's higher malleability. Gemma shows an extreme $Y$-axis shift of -2.3 and an $X$-axis shift of -1.0 in the legal domain. In fact, Gemma consistently demonstrates high cross-domain volatility, with $Y$-axis shifts ranging from -1.1 to -2.3 despite the steering being targeted solely at the $X$-axis. In contrast, Qwen exhibits a domain-resistance effect, or rather internal conflicts. While the workplace domain shifts toward Self-expression (+0.15), the legal domain drifts toward Survival values (-0.22). These opposing reactions result in a neutralized aggregate $X$-shift of only -0.0013, suggesting that Qwen's professional and legal latent structures are governed by discordant internal logic. As expected, Llama remains the most stable, with $X$-axis shifts tightly clustered between -0.17 and -0.26. This uniformity once again indicates that while Llama is harder to move, its cultural priors are more globally consistent across different social contexts than the volatile, domain-sensitive architectures of Gemma and Qwen. \emph{Overall, these findings suggest that activation steering can effectively modify latent cultural states, but precise cultural alignment must account for how different models partition social domains during pre-training.}

To localise hybrid gains across social contexts, we re-run the above domain breakdown under hybrid Setup~1 ($v_L$) and report a per-axis \emph{gap-closure ratio}. For each (model, domain, target country) triple and each axis $a \in \{X, Y\}$, we define
\[
\rho_a \;=\; \frac{s_a - b_a}{h_a - b_a},
\]
where $b_a$ is the unsteered base coordinate, $s_a$ the steered coordinate, and $h_a$ the human baseline on axis $a$. Thus $\rho=1$ closes the gap exactly, $\rho=0$ indicates no movement, $\rho>1$ overshoots, and $\rho<0$ moves away from the target. We use the per-country optimal coefficient adopted elsewhere in this paper. Setup~1 and Setup~2 yield qualitatively similar domain patterns, so we report Setup~1 here and omit Setup~2 for brevity.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{charts/Hybrid_setup_domain_heatmap.png}
    \caption{Per-domain gap-closure ratio $\rho$ under hybrid Setup~1, for each (model, target country) on the $X$-axis (Survival vs.\ Self-Expression) and $Y$-axis (Traditional vs.\ Secular-Rational). Cells are centred at $\rho=1$ (exact closure); $\rho<0$ indicates motion away from the target.}
    \label{fig:hybrid_domain_heatmap}
\end{figure}

The domain-resolved view both sharpens and complicates the aggregate hybrid story of Section~\ref{subsec:hybrid_results}. At the aggregate (\emph{All}) level, the architecture ranking from Figure~\ref{fig:reproduced_map} is preserved: on non-Western targets Qwen closes $\rho_X, \rho_Y \in [0.77, 1.16]$, Gemma reaches $\rho \in [0.33, 0.92]$, and Llama remains bounded at $\rho \le 0.53$ on both axes.

A qualitatively different pattern emerges for Gemma on Denmark. Across all three social domains, $\rho_X$ is negative ($-0.40$ to $-0.17$): hybrid steering \emph{repels} the model from the Danish Survival--Self-Expression target rather than attracting it. Yet the Traditional--Secular-Rational axis tells the opposite story, with $\rho_Y$ positive throughout ($0.22$ to $0.54$). This axis-selective repulsion is itself a signature of latent entanglement: the two cultural axes are not independently steerable for this (model, country) pair, and no choice of domain framing decouples them. It also accounts for the only non-significant distance reduction in Appendix~\ref{app:l2_distance}.

Beyond this anomaly, a domain asymmetry surfaces in the overshoot regime. Whereas \emph{Workplace} was the most resistant partition under pure vector steering, under hybrid Setup~1 it is the \emph{Legal} domain that most aggressively exceeds exact closure: Qwen on Vietnam ($\rho_X{=}1.10$, $\rho_Y{=}1.15$), Qwen on Mexico ($\rho_X{=}1.16$), and Gemma on India ($\rho_Y{=}1.06$) all overshoot, while Workplace remains comparatively moderate. One possible explanation is that the advanced prompt conditioning binds more tightly to legal-context activations than to professional-norms activations, but verifying this would require a separate analysis of prompt--activation interactions.

Llama, by contrast, exhibits uniform rigidity rather than domain-specific resistance. With the exception of Denmark on the $Y$-axis (where Family at $\rho_Y{=}0.48$ contrasts sharply with Legal at $\rho_Y{=}0.02$), the per-domain spread for a given country is narrow and no cell exceeds $\rho{=}0.53$. This suggests that Llama's resistance to hybrid steering reflects model-level properties rather than the particular social framing of the stimuli, consistent with the findings reported in Section~\ref{sec:entanglement} and the vector-steering domain results above. Having characterized the robustness of cultural steering across social domains, we turn to its effect on general reasoning capabilities.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{charts/model_perplexity.png}
    \caption{Perplexity of the LLMs changes when applying vector steering.}
    \label{fig:model_perplexity}
\end{figure}

\subsection{Impact of Cultural Steering on Task Performance}
\label{subsec:mmlu_performance}

To evaluate whether cultural steering preserves general reasoning capabilities, we measure performance on a stratified subset of 1k samples from the \textbf{Global-MMLU} benchmark \cite{DBLP:conf/acl/SinghRFANVLMLSN25}, uniformly sampled across culturally-agnostic (CA), culturally-sensitive (CS), and general knowledge categories. Results per treatment are averaged across the four countries.

\input{tables/mmlu}

Figure~\ref{fig:model_perplexity} shows that perplexity remains near baseline at $\alpha=0.2$ and rises moderately at $\alpha=0.4$, confirming that the performance decreases in Tab.~\ref{tab:mmlu_results} arise from cultural steering rather than linguistic degradation. Cultural steering introduces a consistent but moderate performance decrease that scales with intervention intensity, and the per-model magnitudes echo the steerability ranking established in earlier sections. Gemma, the most malleable architecture, also pays the largest tax, dropping $7.8$ percentage points under Hybrid~2 ($0.608 \to 0.530$); Qwen, the most compositional, loses only $3.0$ points ($0.734 \to 0.704$); and Llama, the most rigid, is the least disturbed and is actually nudged \emph{upward} by Advanced Prompt steering ($0.585 \to 0.598$). Performance on CS and CA subsets closely follows the overall trends, indicating that steering effects are broadly distributed rather than specific to culturally-relevant questions. These results hint at a mild \emph{alignment--capability trade-off}: models that undergo larger cultural shifts also exhibit greater performance degradation, consistent with prior findings \cite{DBLP:journals/corr/abs-2603-18507}. Yet even under the strongest interventions, all models retain sufficient accuracy to maintain cultural alignment without critically compromising task effectiveness.

\paragraph{Summary.} Vector steering reaches culturally diverse coordinates that prompt-only conditioning cannot, particularly for non-Western targets on rigid architectures such as Llama. Hybrid steering further closes the gap on every model--country pair except Gemma on Denmark, and additionally reduces entanglement on the most rigid model. The cost is a bounded, predictable accuracy drop that scales with architecture-specific steerability rather than with the cultural distance traveled. Latent entanglement---the systematic coupling of the Traditional vs.\ Secular-Rational and Survival vs.\ Self-Expression axes---persists across all methods and is the central limitation we carry into Section~\ref{sec:limitations}: it mirrors a genuine $r{=}0.474$ coupling in human WVS data, but it also bounds the precision with which any single-vector intervention can target a specific cultural coordinate.

==> sections/introduction.tex <==
\section{Introduction}
% The global proliferation of Large Language Models (LLMs) has introduced a transformative capacity for cross-cultural communication and decision support. However, as these models are increasingly integrated into social infrastructures—ranging from legal drafting to personal counseling—a fundamental challenge arises regarding the \textit{Western-centric} bias. Most state-of-the-art models are trained on massive web-scale corpora dominated by English-language and Western-centric perspectives, therefore models align primarily with the values of Northern European societies \cite{Tao_2024,zhou2025weird}. This shift risks the systemic homogenization of diverse cultural perspectives, where the unique nuances of local belief systems are eroded in favor of a singular, globally dominant standard \cite{yu2025entangled}.

% While social science frameworks like the World Values Survey (WVS) \cite{WVS_AllRounds,WVS_Wave7} and the European Values Study (EVS) \cite{EVS} provide a gold standard for mapping human values, directly applying these instruments to LLMs presents significant methodological hurdles. Firstly, \textit{Direct explicit prompting} using wvs question often fail to capture a model's latent cultural depth, as they frequently trigger safety-aligned refusals or default to neutral, ``AI-style'' responses. Secondly, recent research suggests that this phenomenon is driven by an \textit{explicit-implicit localization gap} \cite{argin2025localized}, in which models possess latent cultural knowledge that remains inaccessible via standard prompting alone. Lastly, direct survey queries are unable to capture how LLMs manifest values in practical, real-world applications and the variation perspective between domains. Different architectures exhibit varying levels of ``anchoring'' to their training priors, making a universal alignment strategy difficult to implement \cite{zhou2025weird}

The training of Large Language Models (LLMs) on massive English-language web corpora has led to a documented phenomenon of homogenization, where model outputs disproportionately align with the values of Northern European and English-speaking societies \cite{Tao_2024, zhou2025weird}. When evaluated against gold-standard sociological frameworks like the World Values Survey (WVS) \cite{WVS_AllRounds} or the European Values Study (EVS) \cite{EVS},  model default internal priors often collapse toward a singular, dominant standard \cite{yu2025entangled}.

As standard evaluation often relies on direct, explicit prompting, asking models survey questions frequently triggers safety-aligned refusals (e.g., ``I have no personal beliefs'') or anchors responses to a ``neutral'' baseline \cite{argin2025localized}. Furthermore, current methods fail to account for domain-specific variance; a model might respond with Western-centric values in a legal context while retaining country-specific norms in familial settings. Because different architectures exhibit varying levels of ``anchoring'' to their training priors, existing prompt-based alignment strategies are often brittle, resulting in stereotypical personas that fail to capture the model’s internal decision-making.

\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.75\textwidth]{latex//images/evaluation_flow.png}
    \caption{Comparison of cultural evaluation paradigms. The direct explicit prompting (left) often triggers safety refusals or neutral personas, leading to a loss of cultural data. Our proposed scenario-based behavioral probing (right) translates abstract WVS questions into situational dilemmas. By extracting raw logit probabilities, we bypass surface-level personas to map the model's latent coordinates onto the Inglehart-Welzel Cultural Map.}
    \label{fig:evaluation_flow}
\end{figure*}

To address the above limitations, we propose a generalizable framework. Our study examines how effectively the LLMs can be steered with respect to country-specific cultural values, moving from surface-level instructions to latent interventions. We prototype our framework on smaller, open-source LLMs (e.g., Qwen-3-4B-Instruct, Llama-3.2-3B-Instruct, Gemma3-4B-it) to demonstrate its efficacy in shifting internal value alignments without costly retraining. Our contributions are organized into the following two dimensions.

First, to address the limitations of abstract surveys, we developed a dataset that translates WVS value dimensions into 600 situational scenarios (300 for training, 300 for evaluation). For example, the human survey question ``How important is God in your life? (1-10)'' is converted into a scenario: ``Your company is considering replacing religious holidays with elective holidays. Do you support (option A) or oppose (option B) the new policy?'' These scenarios are distributed across three distinct domains, namely family, workplace, and legal, capturing the spectrum of informal social norms and formal institutional rules \cite{North_1990}. 
% This dataset serves as the foundation for our evaluation.
% , enabling the model to move from self-reported beliefs to practical behavioral choices.

Second, we use this dataset to extract cultural coordinates via token-probability analysis. This probing strategy (as outlined in Figure \ref{fig:evaluation_flow}) is directly coupled with a latent intervention using activation steering, allowing us to shift a model's cultural center during the forward pass. To quantify these shifts, we introduce the \textit{entanglement ratio} ($E$), which measures the degree to which cultural axes are coupled within the latent space.

% We compare our method with 2 prompt-based techniques: \textit{basic prompt steering}, which utilizes simple system prompt instructions for the model to adopt a national persona, and \textit{advanced prompt steering}, which provides more detailed cultural priors and value-prioritization instructions. 
We select four target nations representing diverse clusters on the Inglehart-Welzel Cultural map \cite{joint_wvs_evs}: India, Vietnam, Mexico, and Denmark. We evaluate this framework across the 4 nations on 3 models (Llama, Qwen, and Gemma) using multiple configurations. Our experiments reveal that cultural adaptability is not uniform. We see a significant disparity in architectural sensitivity: while Llama exhibits high structural rigidity to steering, Qwen and Gemma demonstrate high volatility, requiring situational context to prevent overshooting into extremes. Finally, our findings on latent entanglement reveal that LLMs encode and internalize sociological dependencies as a monolith rather than as decoupled independent axes, providing critical validation of empirical human data \cite{inglehart2000modernization}.

==> sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}
% While this work establishes a viable framework for cultural intervention through activation steering, several limitations remain. A primary technical challenge identified is \textit{latent entanglement}, where steering along a single axis often unintentionally affects the coordinates of the other cultural dimension. Because this study tested both axes of the World Values Survey (WVS) map, we observed that the effectiveness of the intervention is not uniform; the steering impact varies significantly depending on the specific value-based questions being evaluated. 

% This suggests that future research should move beyond linear vector addition toward multi-step or adaptive steering frameworks \cite{zhao2025bodes, wang2025act} to achieve more precise alignment.

% Furthermore, while our behavioral probing focused on cultural value extraction, it is essential to evaluate how these latent interventions affect general model performance. Future studies should test the impact of activation steering on standard LLM benchmarks and general reasoning tasks to ensure that shifting a model's cultural center does not degrade its broader capabilities or linguistic fluency. 

% Lastly, a significant limitation of the current WVS framework is its reliance on general-purpose indicators. Our findings regarding \textit{Domain Resistance} suggest that these broad questions are often unable to fully reflect the nuances of human values within specific situational contexts, such as the legal or workplace domains. Future research should aim to develop more granular, domain-specific culture maps that can capture the professional and situational complexities that general surveys currently overlook.

While this work establishes a viable framework for cultural intervention and evaluation, several limitations remain. First, the challenge of latent entanglement represents a trade-off between sociological accuracy and alignment precision. While the coupled shifts validate that the model has internalized the correlation observed in human societies, they prevent the independent, orthogonal manipulation of specific cultural dimensions. This suggests that for these architectures, ``Modernity'' is encoded as a monolithic latent feature, limiting the granularity of targeted value interventions. 

Secondly, the current study does not employ the Individualism vs. Collectivism axis, which often correlates with the Traditional vs. Secular-Rational and Survival vs. Self-Expression values. However, in sociological reality, these values exist on a complex, non-linear spectrum where individuals may exhibit collectivist behaviors in familial contexts while remaining highly individualistic in professional environments. Our linear vector steering approach may fail to capture these multifaceted nuances.

Third, using a country as a proxy for culture is an inherent oversimplification. National-level averages from the WVS may overlook the diverse subcultures and transnational identities present within the training data. This ``East-West'' divide fails to account for the significant intra-national variance that exists in real-world sociological data.

\textcolor{red}{Lastly, our findings on domain resistance confirm that general-purpose indicators do not fully reflect the complexities of the legal or workplace domains. Furthermore, we have not yet evaluated the ``alignment tax'', whether these latent interventions degrade general reasoning capabilities or linguistic fluency on standard LLM benchmarks. Future work must investigate the impact of high-intensity steering on broad model utility.}

\textcolor{green}{Finally, our findings on domain resistance confirm that general-purpose indicators do not fully reflect the complexities of the legal or workplace domains. Although we provide an initial assessment of the alignment--capability trade-off through perplexity monitoring and Global-MMLU evaluation (Section~\ref{subsec:mmlu_performance}), these measures offer only a surface-level view of model utility under steering: perplexity captures fluency degradation but not higher-order reasoning failures, and multiple-choice benchmarks may underestimate capability loss on generative or open-ended tasks. Future work should evaluate steered models on a broader suite of capabilities, including chain-of-thought reasoning, instruction following, and domain-specific tasks, particularly under high-intensity steering.}

==> sections/methodology.tex <==
\section{Methodology}
\label{method}

%To investigate the latent cultural dynamics of LLMs, we propose a framework that transitions from passive evaluation to active intervention. 
Our methodology is grounded in the realization that surface-level text generation often masks a model's true value alignment due to safety-guardrails and linguistic desirability. Consequently, the proposed pipeline consists of: (1) construction of a domain-stratified behavioral dataset, (2) application of probability-based token probing to uncover implicit cultural biases, and (3) deployment of selective activation steering to shift the model's latent coordinates. As described in Figure \ref{fig:evaluation_flow}, the workflow allows us to quantify not only where a model sits on the Inglehart-Welzel cultural map but also the extent to which its internal value priors can be reconfigured across different social contexts.

\subsection{Behavioral Dataset Generation}
\label{sec:data_gen}
\color{green}
Direct, survey-style probing measures stated preferences, not latent value priors. Explicit prompts elicit safety-alignment refusals and homogenized responses \cite{DBLP:conf/emnlp/AdilazuardaLGA25}; Likert-style self-report shifts with paraphrase and skews toward socially desirable answers, whereas forced-choice formats produce more stable measurements and better discriminate between models \cite{DBLP:conf/acl/LiSYTZ25,DBLP:conf/nips/Dominguez-Olmedo24,DBLP:conf/emnlp/KabirAA25}. Beyond NLP, Situational Judgment Tests embed values in concrete scenarios rather than abstract rating items and report higher content and criterion validity for behavioral dispositions; intercultural SJTs measure cultural value orientations specifically \cite{rockstuhl2015putting}. fMRI studies of moral judgment locate the neural signature that predicts a participant's choice in scenario-grounded dilemmas, not in abstract rating tasks \cite{greene2001fmri}. Activation steering operates on internal representations; eliciting those representations requires the format that recruits them. We therefore developed a behavioral dataset comprising 600 situational scenarios.
\color{black}
 
 Each sample is structured to include a situational dilemma and two distinct options representing opposite cultural values (e.g., Traditional vs Secular-Rational and Survival vs Self-Expression). For example, the human survey question ``How important is God in your life? (1-10)'' is converted into a scenario: ``Your company is considering replacing religious holidays with elective holidays. Do you support (option A) or oppose (option B) the new policy?'' We categorize our scenarios into three distinct domains: family, workplace, and legal to represent a comprehensive cross-section of the private, professional, and public spheres of human existence. This selection is grounded in the Social Institutional framework \cite{North_1990}, which posits that cultural values manifest differently across varying levels of social distance. By using these three distinct domains, we can evaluate LLMs' default preferences across the informal, high-nuance environment of the family, the standardized, corporate-aligned workplace, and the rule-bound legal domain\footnote{We acknowledge that converting complex sociological questions into binary forced-choice dilemmas involves inherent trade-offs. In domains such as the legal or workplace spheres, choices are often constrained by state jurisprudence or corporate policy rather than personal value alignment alone. %Consequently, mapping these variables to binary tokens necessarily strips away procedural and structural nuances—such as specific national laws on abortion or homosexuality—that would otherwise influence decision-making in real-world institutional contexts.
}. 
%This approach ensures that our analysis captures the full spectrum of the Inglehart-Welzel cultural map while avoiding the safety-trigger noise often found in more polarizing domains such as religion or politics.

We utilized Gemini-2.5-Flash as the base model to generate these dilemmas. For each of the 10 core World Values Survey (WVS) questions (Table~\ref{tab:wvs_dimensions}), we initially generated a larger pool of candidate scenarios in English. We shortlisted the top 20 scenarios per question based on two criteria: (1) contextual relevance, ensuring the dilemma directly forced a choice along the specific WVS axis, and (2) variance maximization, selecting scenarios that presented the most diverse situations.
% to ensure the model's cultural latent features were tested against a wide range of linguistic triggers. 
The final dataset consists of 600 samples (200 per domain), split into 300 for vector optimization $\mathcal{D}_{\textit{train}}$ and 300 for evaluation $\mathcal{D}_{\textit{test}}$. The 300 evaluation items in $\mathcal{D}_{\textit{test}}$ were independently audited by two human annotators and Opus 4.7 against three criteria---domain/topic alignment, neutrality between the two options, and realism of the dilemma; full inter-annotator agreement statistics are reported in Appendix~\ref{sec:verification}.

% To evaluate the impact of language on cultural values, we translated the WVS questions and the 600 generated scenarios into the national languages of the evaluated countries (e.g., Vietnamese, Spanish, Hindi). We employed the NLLB-200 model \cite{nllbteam2022languageleftbehindscaling} for this task ensuring that any observed shifts in cultural output were due to language-specific latent representations rather than translation artifacts.
\color{black}

\subsection{Evaluation via Token Probing}
% To measure the model's latent cultural position, we utilize a probability-based probing framework \cite{choenni-etal-2024-echoes} to explore cultural nuances that standard benchmarks might overlook. This method bypasses the neutral bias often elicited in instruction-tuned models such as \textit{Gemma 3} or \textit{Llama 3.2} - by extracting raw logit probabilities rather than generated text. For each scenario, we present a situational prompt:

To measure the model's latent cultural position, we utilize a probability-based probing framework \cite{DBLP:conf/acl/ChoenniLS24}, extracting logit probabilities rather than generated text. For each scenario in $D_{test}$, we present a situational prompt as described below.

\begin{equation}
\boxed{
\begin{aligned}
\text{\{situation\}}\\
\text{Option A: \{option A\}}\\
\text{Option B: \{option B\}}\\
\text{What will you do (A/B)?}
\end{aligned}
}
\label{eq:situation_prompt}
\end{equation}

To mitigate positional bias, we randomly assign the cultural values (e.g., Traditional vs. Secular-Rational) to either ``Option A'' or ``Option B'' for every trial. After the forward pass, we extract the logits for the tokens `A' and `B' at the last layer and map them back to their corresponding cultural values based on the randomization key. We quantify the model's position along the cultural axis by calculating the softmax probability. Let $z_{pos}$ represent the logit for the positive axis (e.g., Secular-Rational/Self-Expression) and $z_{neg}$ represent the logit for the negative axis (e.g., Traditional/Survival), then score $P$ is defined as (Equation \ref{eq:prob_softmax}). Here, $P \in [0, 1]$, where a score of $1.0$ indicates a total alignment with the positive axis and $0.0$ indicates total alignment with the negative axis. These scores are averaged across all scenarios within a domain and rescaled to the original WVS question ranges for visualization on the 2-D cultural map.
\begin{equation}P = \text{Softmax}(z_{\textit{pos}}) = \frac{e^{z_{\textit{pos}}}}{e^{z_{\textit{pos}}} + e^{z_{\textit{neg}}}} \label{eq:prob_softmax}\end{equation}
The natural language in our prompting setup can also be enhanced by incorporating country-specific cultural information via the system prompt $S$ before the situational prompt (Equation \ref{eq:situation_prompt}). We operationalize this cultural steering via:
\begin{itemize}[itemsep=0pt, topsep=0pt]
    \item \textbf{Basic setup ($S=S_{\textit{basic}}$):} We instruct the model to adopt a national identity \cite{DBLP:journals/corr/abs-2311-14096,DBLP:conf/emnlp/MasudSH0024} (e.g., ``You are a person living in <country>"). This method relies exclusively on the model’s internal, pre-trained associations with the target country (India, Vietnam, Mexico, or Denmark) without providing any explicit value-based guidance.
    \item \textbf{Advanced setup ($S = S_{\textit{advanced}}$):} Here, we construct cultural profiles by first calculating the average numerical response across all survey participants in a target country for each WVS variable. We then identify the specific categorical answer for each question whose index is closest to this country-level mean. Finally, we extract the verbatim answer descriptions from the WVS codebook for these categories and synthesize them into a structured prompt. This process ensures that the personas are grounded in the empirical statistical modes of the target population. To maintain representative naming, we assign high-frequency national names for each country \cite{DBLP:conf/emnlp/PawarAKA25}. Detailed templates are provided in Appendix~\ref{sec:steer_prmopt}.
\end{itemize}

% \color{black}
% \subsection{\color{red}Cultural Value activation steering}
% We formalize cultural alignment as a selective inference-time intervention. Unlike supervised fine-tuning (SFT) \cite{} or Direct Preference Optimization (DPO) \cite{}, which modify the model's underlying parameters $\theta$, steering operates on a frozen model. 

% Prompt-Based Steering (Baseline) is a natural-language intervention that instructs the model to adopt a specific cultural identity via its system prompt. We evaluate two levels of instructional complexity within this paradigm. First, Basic Prompt Steering employs a minimalist instruction that directs the model to adopt a national persona (e.g., ``You are a person living in Vietnam"). This approach relies exclusively on the model's internal, pre-trained knowledge of the target culture, without providing external context. Second, Advanced Prompt Steering provides detailed cultural priors and explicit value-prioritization instructions. In this setting, we test the model's ability to adapt to specific knowledge derived from the target country's actual coordinates on the Inglehart-Welzel Cultural Map. For these experiments, we selected four target nations, namely India, Vietnam, Mexico, and Denmark, that represent distinct clusters on the map \cite{joint_wvs_evs}. Detailed prompt templates for each country and steering level are provided in Appendix \ref{sec:steer_prmopt}.

% \subsection{Prompt-Based Alignment}
% Before investigating latent interventions, we evaluate cultural alignment through natural language prompting. Unlike parameter-efficient methods that modify the model's weights $\theta$, this approach operates on a frozen model, guiding its inference via the system prompt before the situational prompt. We categorize these interventions into two levels of complexity.



% Advanced Cultural Steering: 
% \color{red}
% To evaluate the model’s capacity for deeper alignment, we provide detailed cultural priors \cite{masud-etal-2024-hate}. These are formulated by synthesizing core sociological constructs—such as Filial Piety ($Hi\hat{e}u$) in Vietnam, Personalismo in Mexico, or the Jante Law in Denmark—extracted from the target country’s coordinates on the Inglehart-Welzel Cultural Map \cite{WVS_AllRounds}. To ensure these descriptions are sociologically grounded, we identified the statistical modes of the target population's values in the World Values Survey (WVS) and mapped them into a structured social identity narrative. We also assign personal names for each target country from high-frequency datasets to achieve representative naming \cite{pawar-etal-2025-presumed}. Detailed templates for the four target nations (India, Vietnam, Mexico, and Denmark) are provided in Appendix \ref{sec:steer_prmopt}.
% \color{green}
% To evaluate the model’s capacity for deeper alignment \cite{masud-etal-2024-hate}, we implement cultural profiles derived from the World Values Survey (WVS) \cite{WVS_Wave7}. We construct these profiles by first calculating the average numerical response across all survey participants in a target country for each WVS variable. We then identify the specific categorical answer for each question whose index is closest to this country-level mean. Finally, we extract the verbatim answer descriptions from the WVS codebook for these categories and synthesize them into a structured prompt. This process ensures that the steering vectors ($v$) are grounded in the empirical statistical modes of the target population. To maintain representative naming, we assign high-frequency national names for each country following \cite{pawar-etal-2025-presumed}. Detailed templates for the four target nations (India, Vietnam, Mexico, and Denmark) are provided in Appendix \ref{sec:steer_prmopt}.
% \color{black}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{wvs_zoom.png}
%     \caption{Comparative analysis of cultural map under different evaluation paradigms. (Left) Evaluation using direct explicit prompting. (Right) Evaluation using situational dilemmas reveals a more pronounced latent shift across cultural axes than does clustering in direct questioning.}
%     \label{fig:reproduced_map}
% \end{figure*}
\subsection{Activation Steering Based Alignment}
Our initial experiment with prompt-based steering reveals a gap in the models' steerability. We therefore go a step further, employing activation steering that directly intervenes on the model's latent representations during the forward pass via two empirical steps.

\paragraph{Scenario-based contrasts} Formally, we represent the model's hidden state at layer $L$ as a vector $h_L \in \mathbb{R}^d$ and apply a linear shift to these activations during forward pass. Given a steering vector $v_L$ derived from the contrastive pairs ($a_L^{+}$, `$a_L^{-}$), and a scaling coefficient $\alpha$, the modified hidden state $h_L'$ is defined below as:
\begin{equation}
\begin{aligned}
h_L' = h_L + \alpha v_L \\
v_L = \frac{1}{n} \sum_{i=1}^{n} (a_{i,L}^{+} - a_{i,L}^{-})
\end{aligned}
\label{eq:layer_steering}
\end{equation}

To extract steering vectors ($v_L$) in Equation \ref{eq:layer_steering},we utilize the Dialz framework \cite{DBLP:conf/acl/SiddiqueTA25}. 
While Dialz proposes two extraction methods, namely Principal Component Analysis (PCA) and ``mean difference'', we employ the latter, as our initial empirical testing demonstrated a stronger steering effect on cultural alignment. Here, $n$ represents the total number of contrastive samples used to compute the directional vector.
We generate contrastive text input pairs by decoupling and linearizing the situational probe in Equation \ref{eq:situation_prompt} for situations in $D_{train}$ as follows:
% \begin{equation}
% \boxed{
% \begin{aligned}  
% a_L^{+}=\text{\{situation\}} + \text{ \{option A\}} \\
% a_L^{-}=\text{\{situation\}} + \text{ \{option B\}}. 
% \end{aligned}
% }
% \label{eq:situation_constrast}
% \end{equation}

\begin{equation}
\boxed{
\begin{aligned}  
a_L^{+} &= f_L(\text{situation} + \text{option A}) \\
a_L^{-} &= f_L(\text{situation} + \text{option B}) 
\end{aligned}
}
\label{eq:situation_constrast}
\end{equation}

Thus,  $a_L^{+}$ and $a_L^{-}$ in Equation \ref{eq:situation_constrast} are the activations at layer $L$ elicited by the contrastive prompts representing positive (Secular-Rational/Self-Expression) and negative (Traditional/Survival) cultural anchors, respectively. It is important to note that at this stage, the contrastive pairs are formulated in neutral, value-based language, without any country-specific identifiers or personas. Consequently, the resulting vector $v_L$ represents a general direction in the latent value space that remains identical across all target countries before any further conditioning is applied.

% To extract these vectors, we utilize the Dialz framework \cite{siddique-etal-2025-dialz}, following a systematic three-step pipeline designed including Vector Extraction, Layer-wise Grid Search, and Multi-Layer Cultural Intervention to identify and apply cultural value directions.

% First, for each cultural axis, we provide the model with contrastive prompt pairs consisting of a situational dilemma followed by a culturally-aligned action (e.g., a ``Traditional'' action vs. a ``Secular-Rational'' action). We calculate the steering vector $v$ at each layer $L$ as the mean difference in the activation scores between these contrastive sets:
% \begin{equation}v_L = \frac{1}{n} \sum_{i=1}^{n} (a_{i,L}^{+} - a_{i,L}^{-})\end{equation}
% where

\paragraph{Layer-selection heuristics} 
Existing literature has highlighted that the efficacy of steering and probing is highly sensitive to the layers in question \cite{DBLP:conf/acl/SiddiqueTA25,DBLP:conf/eacl/MasudKGAC24}. We also hypothesize that applying $v$ to all layers can degrade the model's linguistic coherence. We therefore introduce an empirical selection step based on the shift in model output. Specifically, for each layer $l$, we apply the steering transformation defined in Equation \ref{eq:layer_steering} to the activations $h_l$ with $\alpha=0.2$. We then measure the resulting change in the probability $P$ for situations in $D_{train}$, the likelihood of a culturally aligned response as defined in Equation \ref{eq:prob_softmax}.  
By performing this layer-wise search, we isolate the specific layers where the model's cultural decision-making logic is most densely encoded.
% \textcolor{red}{Following the grid search, we identify the four layers that yield the most significant behavioral shift and aggregate them into the final intervention to maintain overall coherence.}
The resulting steering differentials exhibit a sharp exponential decay across layers (Figure~\ref{fig:layer_selection}), with the top four layers capturing the steep portion of this curve before marginal gains become negligible. Crucially, these top-ranked layers are also the most consistent across individual WVS questions, forming tight clusters regardless of the specific cultural dimension being steered. We therefore aggregate these four layers into the final intervention, as extending beyond this point yields diminishing returns while increasing the risk of interference across unrelated representational functions.

For pure vector steering, we search $\alpha \in [-0.3, 0.6]$; negative values 
steer in the opposing cultural direction, confirming that $v_L$ encodes a 
reversible bidirectional axis in the latent space (Figure \ref{fig:steering_culture_map}).

% This ensures a high-precision shift in cultural trajectory while maintaining the model’s general generating capabilities and linguistic fluency.
\subsection{Hybrid Steering: Combining Latent Activation and System Prompting}
\label{subsec:hybrid_steering}

To investigate the interaction between internal hidden states and external textual instructions, we propose a hybrid steering framework. This approach integrates activation steering with system-level prompting to evaluate whether latent interventions can reinforce or override the model's surface-level cultural alignment.

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{charts/wvs_2.png}
    \caption{Cultural value alignment across steering paradigms on the Inglehart-Welzel Cultural Map. The leftmost panel shows evaluation via direct explicit WVS prompting; the remaining three panels show scenario-based behavioral probing results for Qwen, Llama, and Gemma, respectively. Arrows indicate the trajectory from the model's default coordinates to the steered position for each target country under five configurations: default (grey), basic prompt (purple), advanced prompt (orange), hybrid Setup~1 with base vector + advanced prompt (green), and hybrid Setup~2 with prompt-informed vector + advanced prompt (red). Bottom bar charts display the Euclidean distance from empirical human WVS coordinates; lower values indicate closer cultural alignment.}
    \label{fig:reproduced_map}
\end{figure*}

\paragraph{\textbf{Hybrid Configurations}}
We explore two distinct setups to integrate a system prompt $S$ into the steering process. These configurations aim to clarify whether the ``cultural direction'' remains consistent when the model is already conditioned by a specific cultural persona.

\paragraph{\textbf{Setup 1: Post-hoc System Prompting}}
In this configuration, we utilize the base steering vector $v_L$ (extracted from neutral situational dilemmas without any system prompt) and apply it while the model is provided with a system prompt $S$. The intervention is formulated as follows:

\begin{equation}
h_L' = h_L(S) + \alpha v_L
\end{equation}

where $h_L(S)$ represents the model's hidden state at layer $L$ when processing the test dilemma $D_{test}$ under the influence of system prompt $S$. This setup tests the additive effect of a general latent vector on a model already guided by explicit instructions.

\paragraph{\textbf{Setup 2: Prompt-Informed Vector Extraction}}
In the second configuration, we derive a specialized steering vector $v_L^{sp}$ by extracting activations from contrastive pairs that are already conditioned by the system prompt $S$. The prompt-informed vector is defined as:

\begin{equation}
\begin{aligned}
v_L^{sp} &= \frac{1}{n} \sum_{i=1}^{n} (a_{i,L}^{+, S} - a_{i,L}^{-, S}) \\
a_{i,L}^{+, S} &= f_L(S, \text{situation}, \text{option A}) \\
a_{i,L}^{-, S} &= f_L(S, \text{situation}, \text{option B})
\end{aligned}
\label{eq:prompt_informed_vector}
\end{equation}

where $f_L(\cdot)$ denotes the activation at layer $L$ for the concatenated input. The resulting intervention is:

\begin{equation}
h_L' = h_L(S) + \alpha v_L^{sp}
\end{equation}

This setup captures a ``context-aware'' latent direction that directly corresponds to the cultural persona defined in $S$. We evaluate these configurations using the prompt setups defined in Section 3.2, where $S \in \{S_{basic}, S_{advanced}\}$. 



\paragraph{Coefficient Optimization}
Since the trajectory curve traced by $\alpha$ is architecture- and country-dependent, fixing a single coefficient for all targets risks either undershooting or overshooting the target cultural coordinates. We therefore adopt a two-stage procedure to find the optimal coefficient while avoiding data leakage. In the first stage, we extract a preliminary steering vector using 180 samples from $D_{train}$ and evaluate it across the remaining 120 held-out samples to perform a grid search over $\alpha \in [0, 0.6]$. Negative values are 
excluded here since the system prompt $S$ already conditions the model toward 
the target persona; steering in the opposing direction would work against the 
alignment objective in Equation~\ref{eq:alpha_opt}. The upper bound of $0.6$ is determined by two complementary criteria: perplexity degradation (Appendix~\ref{app:exp_setup}) and trajectory saturation, whereby the cultural coordinates exhibit diminishing displacement per unit increase in $\alpha$ and effectively cease to progress beyond this value. Searching further would therefore increase linguistic instability without expanding the reachable region of the cultural map.

\begin{equation}
    \alpha^{*} = \argmin_{\alpha \in [0,\, 0.6]} 
    \left\| \mathbf{c}(\alpha) - \mathbf{c}_{\text{human}} \right\|_2
    \label{eq:alpha_opt}
\end{equation}

where $\mathbf{c}(\alpha) \in \mathbb{R}^2$ denotes the steered cultural coordinates at coefficient $\alpha$ and $\mathbf{c}_{\text{human}}$ denotes the target country's empirical WVS position. In the second stage,we re-extract the final steering vector using the full 300 samples of $D_{train}$ with $\alpha^{*}$ fixed, producing a higher-quality vector that benefits from the complete training pool. This final vector is then applied at evaluation time on $D_{test}$.

Detailed results and cultural coordinate shifts are presented in Section~\ref{subsec:hybrid_results}.


% \begin{figure}[ht]
%     \centering
%     \begin{tikzpicture}
%         \begin{axis}[
%             ybar,
%             cycle list name=Set1-6,
%             width=\linewidth,
%             height=6.5cm,
%             bar width=0.12cm,
%             % Maps the 'metric' column to the X axis
%             symbolic x coords={Total, Culture, CA, CS},
%             xtick=data,
%             ylabel={Accuracy},
%             % Y-axis control: starts at 0.5, steps of 0.02
%             ymin=0.5, ymax=0.66,
%             ytick={0.50, 0.52, 0.54, 0.56, 0.58, 0.60, 0.62, 0.64, 0.66},
%             enlarge x limits=0.2,
%             % Legend configuration: 2 rows of 3 columns
%             legend style={at={(0.5,-0.25)}, anchor=north, legend columns=3, font=\footnotesize},
%             ymajorgrids=true,
%             grid style=dashed,
%             title={Model Performance Grouped by Accuracy Metric},
%             nodes near coords,
%             every node near coord/.append style={rotate=90, anchor=west, font=\tiny, /pgf/number format/precision=2}
%         ]
            
%             % Each column in the transposed CSV becomes one plot (one bar in each group)
%             \addplot table [x=metric, y=Default, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Default}
            
%             \addplot table [x=metric, y={Basic Prompt}, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Basic Prompt}
            
%             \addplot table [x=metric, y={Adv Prompt}, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Adv Prompt}
            
%             \addplot table [x=metric, y={Vec Steer}, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Vec Steer}
            
%             \addplot table [x=metric, y={Hybrid 1}, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Hybrid 1}
            
%             \addplot table [x=metric, y={Hybrid 2}, col sep=comma] {data_transposed.csv};
%             \addlegendentry{Hybrid 2}

%         \end{axis}
%     \end{tikzpicture}
%     \caption{Comparison of accuracy metrics across six experimental configurations, grouped by evaluation category.}
%     \label{fig:performance_grouped}
% \end{figure}


% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{hybrid_basic_method.png}
%     \caption{The results demonstrate that while the hybrid method successfully shifts the model’s latent coordinates toward the intended cultural quadrants, thereby providing a more pronounced alignment than prompting alone, the relative distance between the target countries remains notably small. This high density within the shifted cluster suggests that although the latent intervention effectively moves the model along the "Survival vs. Self-Expression" and "Traditional vs. Secular-Rational" axes, the underlying model priors still exert a form of structural rigidity that limits distinct cultural differentiation when using only basic instructions.}
%     \label{fig:hybrid_basic}
% \end{figure*}

% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{hybrid_advance_method.png}
%     \caption{In contrast to the basic prompting setup, the use of advanced instructions in the Qwen model results in a significantly wider dispersion of cultural coordinates, with each target country moving toward more distinct and specialized positions on the WVS map. However, a notable discrepancy is observed in the Gemma model, which continues to exhibit high density and minimal differentiation between countries despite the more detailed prompt. This suggests that while advanced prompting can unlock greater latent flexibility in certain architectures like Qwen, others remain constrained by a "structural rigidity" that resists divergent cultural alignment even under sophisticated hybrid interventions.}
%     \label{fig:hybrid_advance}
% \end{figure*}

==> sections/relatedwork.tex <==
\section{Related Work}

\paragraph{Cultural Map and Value Dimensions}
The World Values Survey (WVS) \cite{WVS_AllRounds} represents the most comprehensive longitudinal investigation of human values, spanning over 100 countries and involving over 400k participants since its inception in 1981. The survey is conducted in multiple ``waves'' approximately every 5 years.
% allowing researchers to track significant cultural value shifts over time. 
% These temporal shifts—often driven by economic development or generational replacement—underscore the dynamic nature of culture and make the task of LLM alignment particularly urgent; models must not only be culturally aware but also able to reflect the evolving values of the societies they serve.
Part of WVS translates high-dimensional survey responses converted into a two-dimensional visualization known as the Inglehart-Welzel cultural map.
% This is achieved through \textbf{Factor Analysis}, a statistical method that identifies latent variables responsible for the correlations between multiple survey items.
The analysis consistently reveals two dominant dimensions of cross-cultural variation: \textit{Traditional} vs. \textit{Secular-Rational} and \textit{Survival} vs. \textit{Self-Expression}. While the original sociological work focuses on the evolution of these values across decades \cite{EVS2022,WVS2022}, this research focuses on their current/latest state. 
% We focus on aligning models with the contemporary cultural positions identified in the latest waves of the WVS, 
% rather than on addressing the longitudinal value shifts themselves. 
As shown in Figure \ref{fig:reproduced_map}, we have reproduced the cultural map, including the positions of current LLMs.
% (Section \ref{method} for more details).

% Consistent with recent findings \cite{Johnson2022, Adilazuarda2024}, our visualization highlights a pronounced Western-centric skew, with models gravitating toward the Secular-Rational and Self-Expression quadrants. However, recent scholarship critiques the use of WVS as a definitive proxy for cultural alignment. Specifically, studies suggest that LLMs’ survey responses can be highly unstable and sensitive to prompt formatting rather than reflecting true latent values \cite{Bravansky2025, Pezeshkpour2023}. Furthermore, relying solely on WVS dimensions may inadvertently homogenize cultural nuances, as survey data often fails to capture the intricate historical and contextual norms required for downstream tasks such as offensiveness classification \cite{adilazuarda-etal-2025-surveys}. To understand the specific psychological markers measured, Table \ref{tab:wvs_dimensions} lists the cultural values required for each dimension.

Consistent with recent findings \cite{johnson2022mirroring, adilazuarda2024towards}, our visualization highlights a pronounced Western-centric skew, with models gravitating toward the Secular-Rational and Self-Expression quadrants. However, recent scholarship critiques the use of WVS as a definitive proxy for cultural alignment. Specifically, studies suggest that LLMs’ survey responses can be highly unstable and sensitive to prompt formatting rather than reflecting true latent values \cite{bravansky2025break, pezeshkpour2023questioning}. Furthermore, relying solely on WVS dimensions may inadvertently homogenize cultural nuances, as survey data often fails to capture the intricate historical and contextual norms required for downstream tasks such as offensiveness classification \cite{adilazuarda-etal-2025-surveys}. To understand the specific psychological markers, Table \ref{tab:wvs_dimensions} lists the cultural values required to measure each dimension.


\begin{table}[h]
\centering
\small
\begin{tabularx}{\linewidth}{p{1.2cm}Xr}
\toprule
\textbf{Dimension} & \textbf{Core Emphasis} & \textbf{QID} \\
\midrule
Traditional & God is very important in respondent's life. & \textbf{Y01} \\
& Priority on obedience/faith over independence. & \textbf{Y02} \\
(Secular-Rational& Abortion is never justifiable. & \textbf{Y03} \\
is opposite)& Strong sense of national pride. &  \textbf{Y04} \\
& Favors respect for authority.  & \textbf{Y05} \\
\midrule
Survival & Priority on security over self-expression. & \textbf{X01} \\
& Describes self as not very happy. & \textbf{X02} \\
(Self-Expression& Homosexuality is never justifiable.  & \textbf{X03} \\
 is opposite)& Would not sign a political petition.  & \textbf{X04} \\
& Caution regarding trusting people. & \textbf{X05} \\
\bottomrule
\end{tabularx}
\caption{Cultural dimension and corresponding WVS survey question \cite{WVS_AllRounds}. QIDs are internal identifiers where X and Y denote questions contributing to their respective axes; these do not correspond to original WVS variable IDs.}
\label{tab:wvs_dimensions}
\end{table}


\paragraph{Cultural Values Evaluation}
The methodologies used to assess and modify the cultural alignment of LLMs have significant implications for their reliability. \citet{Tao_2024} demonstrated that while proprietary LLMs can achieve increased alignment with target nations through role-play or persona-based steering, their analysis does not visualize where the model is situated within the Inglehart-Welzel cultural map post-intervention. Furthermore, their study omits evaluating open-source models, which are more practical for local deployment. 
%Our experiments with open-source architectures, such as Qwen-3-4B-Instruct, indicate that these models remain heavily anchored to Western cultural defaults regardless of the prompt complexity. This suggests that persona-based steering relies heavily on vast latent pre-training knowledge—a resource that is notably limited in smaller models.
Traditional evaluation, which also relies on direct survey questions, presents significant methodological hurdles. \citet{choenni-etal-2024-echoes} argue that direct questioning often triggers a model's safety alignment or results in ``value bleeding'' across languages \cite{adilazuarda-etal-2025-surveys}. To achieve a deeper understanding of the model's decision-making process, \citet{choenni-etal-2024-echoes} uses a robust probing method to extract the probability of target answer tokens. This allows for a more granular tracing of how values emerge or shift during fine-tuning.
%Similarly, \citet{adilazuarda-etal-2025-surveys} point out that asking LLMs for abstract feelings or survey responses often leads the model to avoid answering or to provide homogenized, neutral responses due to a lack of situational context. They advocate for a transition from surveys to narratives, utilizing scenario-based probes to capture differentiated cultural values.
Our work builds on these insights by moving away from direct survey questions and utilizing a scenario behavioral dataset. By combining scenario-based narratives with the token-probability extraction techniques suggested by \citet{choenni-etal-2024-echoes}, we provide a more robust medium for unveiling cultural nuances that standard benchmarks might overlook.

\paragraph{Cultural Value Adaptation for LLMs}
% Simple approaches to cultural adaptation rely on natural-language instructions, such as ``Persona Prompting'' \cite{Tao_2024,choenni-etal-2024-echoes}, in which a model is asked to adopt a specific cultural identity. 
% However, our experiments identifies a phenomenon in which the specificity and detail of a cultural prompt often result in a higher Euclidean distance from authentic human values in a survey context. This suggests that instructional prompts often trigger superficial stereotypes or conflict with internal safety guardrails, resulting in inconsistent behavior across different cultural dimensions \cite{dammu-etal-2024-uncultured}. Moreover 
Existing work shows that culture adaptation via prompting is strongly influenced by the model's ability to follow instructions and its internal knowledge \cite{Tao_2024,tanwar-etal-2023-multilingual}. Consequently, activation steering has emerged as a promising paradigm for modifying model alignment at inference time without the need for computationally expensive retraining. This method involves identifying a specific ``value direction'' within the model's latent space and updating the hidden states during the forward pass to influence model behavior. Different research efforts have proposed varying strategies for finding optimal steering vectors, leading to a growing body of work, such as the SteerBench framework \cite{chen2025steerbenchbenchmarkevaluatingsteerability}, focused on the general steerability of LLMs. Most recently, the \textit{Dialz} framework was released as a standardized Python toolkit to facilitate the creation, application, and visualization of steering vectors \cite{siddique-etal-2025-dialz}.  While recent literature has successfully applied steering vectors to control specific character personas \cite{anonymous2025persona} and to mitigate common social biases related to race, gender, and socioeconomic status \cite{siddique2025shiftingperspectivessteeringvectors}, to the best of our knowledge, our work is the first to address multidimensional cultural value alignment along the Inglehart-Welzel axes via steering.

% Our empirical observations suggest that the Llama-3.2-3B-Instruct model exhibits higher resistance to cultural prompting—remaining anchored to its internal priors—compared to the Qwen-3-4B-Instruct model. That makes the alignment is unstable and difficult to control if we only rely on prompting. 

% Despite being a robust method that saves significant input tokens compared to complex persona prompting, there is currently no universal ``recipe'' for establishing steering vectors; the process remains an iterative cycle of trial and error. 

% We utilize the \textit{Dialz} framework in this research and introduce a systematic optimization method for cultural steering. Specifically, we propose a workflow that optimizes the steering vector by using a structured set of contrastive responses to ensure the vector captures the true cultural value rather than stylistic noise.

==> tables/name.tex <==
\begin{table}[h]
\centering
\footnotesize
\begin{tabular}{lccc}
\toprule
Configuration & \texttt{Llama} & \texttt{Qwen} & \texttt{Gemma} \\
\midrule
Default          & 0.585 & \textbf{0.734} & \textbf{0.608} \\
Basic Prompt     & 0.587 & 0.718 & 0.593 \\
Advanced Prompt  & \textbf{0.598} & 0.719 & 0.562 \\
Vector Steering  & 0.561 & 0.707 & 0.564 \\
Hybrid~1         & 0.575 & 0.700 & 0.536 \\
Hybrid~2         & 0.567 & 0.704 & 0.530 \\
\bottomrule
\end{tabular}
\caption{Global-MMLU accuracy across steering configurations, averaged over the four target country personas.}
\label{tab:mmlu_results}
\vspace{-12pt}
\end{table}
